Graph Connectivity and Single Element Recovery via Linear and OR Queries

We study the problem of finding a spanning forest in an undirected, $n$-vertex multi-graph under two basic query models. One is the Linear query model which are linear measurements on the incidence vector induced by the edges; the other is the weaker OR query model which only reveals whether a given subset of plausible edges is empty or not. At the heart of our study lies a fundamental problem which we call the {\em single element recovery} problem: given a non-negative real vector $x$ in $N$ dimension, return a single element $x_j > 0$ from the support. Queries can be made in rounds, and our goals is to understand the trade-offs between the query complexity and the rounds of adaptivity needed to solve these problems, for both deterministic and randomized algorithms. These questions have connections and ramifications to multiple areas such as sketching, streaming, graph reconstruction, and compressed sensing. Our main results are: * For the single element recovery problem, it is easy to obtain a deterministic, $r$-round algorithm which makes $(N^{1/r}-1)$-queries per-round. We prove that this is tight: any $r$-round deterministic algorithm must make $\geq (N^{1/r} - 1)$ linear queries in some round. In contrast, a $1$-round $O(\log^2 N)$-query randomized algorithm which succeeds 99% of the time is known to exist. * We design a deterministic $O(r)$-round, $\tilde{O}(n^{1+1/r})$-OR query algorithm for graph connectivity. We complement this with an $\tilde{\Omega}(n^{1 + 1/r})$-lower bound for any $r$-round deterministic algorithm in the OR-model. * We design a randomized, $2$-round algorithm for the graph connectivity problem which makes $\tilde{O}(n)$-OR queries. In contrast, we prove that any $1$-round algorithm (possibly randomized) requires $\tilde{\Omega}(n^2)$-OR queries.

==> graph-warmup-corollaries.tex <==
\begin{lemma}\label{lem:bin-search-cor}
	Given a multigraph $G$, in $r$-rounds and $O(n^{1+\frac{1}{r}})$-\BIS queries per round, we can find an edge incident on every vertex.
\end{lemma}
\begin{proof}
	Apply Lemma~\ref{lem:bin-search} in parallel for every vertex $v$ on the $(n-1)$-dimensional vector $x$ where $x_j$ indicates whether $(v,j)$ is an edge or not.
\end{proof}

Given two vertices $a$ and $b$ it is trivial to decide whether there is an edge between $a$ and $b$ with one \BIS query.
We will be requiring a lifting of this to subsets. In particular given two subsets $A$ and $B$, we would require to find an edge $(a,b)$ with $a\in A$ and $b\in B$. The next lemma shows how to do this.

\begin{lemma}\label{lem:det-set-to-set}
	Let $A$ and $B$ be two {\em disjoint} sets of vertices with at least one edge between them. Then in $2r$ rounds and $O(|A|^{1/r} + |B|^{1/r})$-\BIS queries, we can find one edge $(a,b)$ with $a\in A$ and $b\in B$.
\end{lemma}
\begin{proof}
	Consider the $|B|$ dimensional vector $x$ where $x_b$ indicates the number of edges from a vertex $b\in B$ to vertices in $A$.
	We can simulate an \OR-query in this vector using a \BIS-query in the graph --- for any subset $S\subseteq B$, $\OR(x,S)$ has the same answer as $\BIS(A,S)$. Therefore, using Lemma~\ref{lem:bin-search}, in $r$-rounds and $|B|^{1/r}$-\BIS-queries, we can find a coordinate $b^*\in B$ with $x_{b^*} > 0$. That is, there is an edge between $b^*$ and some vertex in $A$.
	
	We can find one such vertex $a\in A$ to which $b^*$ has an edge, again as above. We define the $|A|$-dimensional vector $y$ where $y_a$ indicates the number of edges from $b^*$ to $a$. Once again, the \OR-query on $y$ can be simulated using a \BIS query on the graph --- for any subset $S\subseteq A$, $\OR(y,S) = \BIS(S,\{b^*\})$. 
\end{proof}

\begin{lemma}\label{lem:det-supp-one-cor}
	Let $A$ and $B$ be two {\em disjoint} sets of vertices with exactly one pair $a\in A$ and $b\in B$ having any edge.
	Then this pair can be found in $1$-round using $O(\log n)$ \BIS-queries.
\end{lemma}
\begin{proof}
	As in the proof of Lemma~\ref{lem:bin-search-cor}, construct the $|B|$-dimensional vector $x$ with $x_b$ equal to the number of edges from $b\in B$ to vertices in $A$. Also construct the $|A|$-dimensional vector $y$ with $y_a$ equal to the number of edges from $a\in A$ to $B$.
	Note for the $\OR$-queries can be simulated in $x$ and $y$, using $\BIS$-queries. Also note that both $x$ and $y$ have {\em exactly} one non-zero entry.
	
	Using Lemma~\ref{lem:det-supp-one}, in one round we can simultaneously find the $a$ and $b$ with $x_a > 0$ and $y_b > 0$. This must be the pair we are looking for.
\end{proof}

\begin{lemma}\label{lem:det-supp-d-cor}
	If a vertex $v$ has degree $\leq d$, then all its neighboring edges can be found in $1$-round in  $O(d^2\log^2 n)$ \BIS-queries or
	$O(d\log^2 n)$ \ADD-queries.
\end{lemma}

\begin{lemma}[An immediate corollary of Lemma~\ref{lem:rand-single-element-recovery}]\label{lem:rand-graph-v-to-S}
	For any vertex $v$ and subset $S\subseteq V\setminus v$, there is a $1$-round randomized algorithm using $O(\log^2 n)$ \BIS-queries which whp returns 
	an edge from $v$ to $S$ if any.
\end{lemma}

\begin{lemma}[A corollary of Lemma~\ref{lem:rand-single-element-recovery}]
	Let $A$ and $B$ be two disjoint subset of vertices in $G$ with at least one edge between them.
	There is a $1$-round randomized algorithm using $O(\log^2 n)$ \OR-queries which  finds an edge in the set $E(A,B)$.
	There is a $2$-round randomized algorithm using $O(\log^2 n)$ \BIS-queries which  finds an edge in the set $E(A,B)$.
\end{lemma}
\begin{proof}
	For the first part, let $x$ be the $|A|\times |B|\leq n^2$ dimensional vector with $x_{ab}$ indicating the number of edges between $a\in A$ and $b\in B$.
	Note that an $\OR(x,S)$ query on this vector for $S\subseteq A\times B$ can be simulated using an $\OR$-query on the graph as well. The rest is implied by Lemma~\ref{lem:rand-single-element-recovery}.
	
	%	We do not know how to simulate the above using $1$-round of \BIS-queries. However, we can simulate using $2$-rounds using similar ideas as in the previous subsection.
	We first consider the $|B|$-dimensional vector $x$ where $x_b$ indicates the number of edges from $b\in B$ to $A$. An $\OR$-query in $x$ can be simulated using $\BIS$-queries.
	Therefore, using the algorithm in Lemma~\ref{lem:rand-single-element-recovery}, we can recover a $b^*\in B$ with $x_{b^*} > 0$. In the next round we construct the $|A|$-dimensional vector $y$ 
	where $y_a$ indicates the number of edges between $a$ and $b^*$. Again using the algorithm in Lemma~\ref{lem:rand-single-element-recovery}, we can recover a $a\in A$ with $y_{a} > 0$.
	That is, $(a,b^*)$ is an edge.
\end{proof}

\begin{lemma}\label{lem:rand-mult-element-recovery}
	If $x\in \RR^N_{\geq 0}$, then there is a $1$-round randomized algorithm using $O(s\log^2 n)$ \OR-queries which returns $s$ random elements in $\supp(x)$ whp.
	Given an upper bound $d$ on $\supp(x)$, there is a $1$-round randomized algorithm using $O(d\log^2 n)$ \OR-queries which recovers $\supp(x)$ whp.
\end{lemma}
\begin{proof}
	Apply the algorithm asserted in Lemma~\ref{lem:rand-single-element-recovery} $s$ times in parallel. For the second part apply coupon collector. {\bf deepc: needs to be completed}.
\end{proof}


\begin{lemma}[An immediate corollary of Lemma~\ref{lem:rand-mult-element-recovery}]\label{lem:rand-graph-sample}
	For any vertex $v$, there is a $1$-round randomized algorithm using $O(s\log^2 n)$ \BIS-queries which, with constant probability, returns $s$ random edges incident on $v$ uniformly at random with repetition.
	There is a $1$-round randomized algorithm using $O(d\log^3 n)$ \BIS-queries which returns all edges incident on $v$ with high probability.
\end{lemma}

\begin{lemma}[A corollary of Lemma~\ref{lem:rand-mult-element-recovery}]\label{lem:rand-graph-cut-vertex-nbrs}
	Let $A$ be a subset of vertices and let $d$ be an upper bound on the number of edges in $E(A,A^c)$.
	There is a $1$-round randomized algorithm using $O(d \log^3 n)$ \BIS-queries which whp finds the subset $B\subseteq A^c$ of vertices 
	which has at least one edge to some vertex in $A$.
\end{lemma}
\begin{proof}
	For the first part, let $x$ be the $|A^c|$ dimensional vector with $x_{b}$ indicating the number of edges between $b\in A^c$ and $A$.
	Note that an $\OR(x,S)$ query on this vector for $S\subseteq A\times A^c$ can be simulated using an $\BIS$-query on the graph as well. Note $\supp(x) \leq d$ (it could be much smaller).
	Using the algorithm asserted in Lemma~\ref{lem:rand-mult-element-recovery}, we can find $\supp(x)$, that is, all $b\in A^c$ which have some neighbor in $A$.
	This is precisely what this lemma asserts.
	
	%	We do not know how to simulate the above using $1$-round of \BIS-queries. However, 
	%	Wwe can simulate using $2$-rounds using similar ideas as in the previous subsection.
	%	We first consider the $|A^c|$-dimensional vector $x$ where $x_b$ indicates the number of edges from $b\in A^c$ to $A$. An $\OR$-query in $x$ can be simulated using $\BIS$-queries.
	%	Note $\supp(x) \leq d$.
	%	Therefore, using the algorithm in Lemma~\ref{lem:rand-mult-element-recovery}, in one round we can recover {\em all} $b^*\in A^c$ with $x_{b^*} > 0$. Let $B := \{b^*\in A^c: x_{b^*} > 0\}$ whp.
	%	That is, every vertex $b^*\in B$ has an edge to some vertex in $A$.
	%	In the next round, 
	%	In the next round we construct the $|A|$-dimensional vector $y$ 
	%	where $y_a$ indicates the number of edges between $a$ and $b^*$. Again using the algorithm in Lemma~\ref{lem:rand-single-element-recovery}, we can recover a $a\in A$ with $y_{a} > 0$.
	%	That is, $(a,b^*)$ is an edge.
\end{proof}

\begin{lemma}[A corollary to Lemma~\ref{lem:rand-supp-estimate}]\label{lem:rand-bis-degree-estimate}
	Let $A$ be a subset of vertices in a graph. There is a $1$-round randomized algorithm which makes  $O(\log^2 n)$-\BIS-queries which returns an estimate $d$ of the $|E(A,A^c)|$ support which whp satisfies $\frac{|E(A,A^c)|}{3} \leq d \leq 3|E(A,A^c)|$.
\end{lemma}


==> macros.tex <==
%%%%%%%%%%

\newcommand{\algline}{
 % \nointerlineskip \vspace{\baselineskip}%
  \rule{0.5\linewidth}{.1pt}\hspace{\fill}%
  \par\nointerlineskip \vspace{.1pt}
}


% General:
\newcommand{\tvd}[2]{\ensuremath{\norm{#1 - #2}_{tvd}}}
\newcommand{\Ot}{\ensuremath{\widetilde{O}}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\Paren}[1]{\Big(#1\Big)}
\newcommand{\Bracket}[1]{\Big[#1\Big]}
\newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\paren}[1]{\ensuremath{\left(#1\right)}\xspace}
\newcommand{\card}[1]{\left\vert{#1}\right\vert}
\newcommand{\Omgt}{\ensuremath{\widetilde{\Omega}}}
\newcommand{\half}{\ensuremath{{1 \over 2}}}

\newcommand{\IR}{\ensuremath{\mathbb{R}}}
\newcommand{\IQ}{\ensuremath{\mathbb{Q}}}
\newcommand{\IIZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\IN}{\ensuremath{\mathbb{N}}}
\newcommand{\IS}{\ensuremath{\mathbb{S}}}
\newcommand{\IB}{\ensuremath{\mathbb{B}}}

\newcommand{\norm}[1]{\ensuremath{\|#1\|}}

\newcommand{\lee}{\leqslant}
\newcommand{\gee}{\geqslant}
\newcommand{\ceil}[1]{{\left\lceil{#1}\right\rceil}}
\newcommand{\floor}[1]{{\left\lfloor{#1}\right\rfloor}}
\newcommand{\prob}[1]{\Pr\paren{#1}}
\newcommand{\expect}[1]{\Exp\bracket{#1}}
\newcommand{\var}[1]{\textnormal{Var}\bracket{#1}}
\newcommand{\eexp}[1]{\exp\paren{#1}}
\newcommand{\set}[1]{\ensuremath{\left\{ #1 \right\}}}
\newcommand{\poly}{\mbox{\rm poly}}
\newcommand{\polylog}{\mbox{\rm  polylog}}

\newcommand{\OPT}{\ensuremath{\mbox{\sc opt}}\xspace}
\newcommand{\opt}{\textnormal{\ensuremath{\mbox{opt}}}\xspace}
\newcommand{\APX}{\ensuremath{\mbox{APX}}}
\newcommand{\apx}{\ensuremath{\mbox{apx}}}
\newcommand{\ALG}{\ensuremath{\mbox{\sc alg}}\xspace}
\newcommand{\alg}{\ensuremath{\mathcal{A}}\xspace}

\DeclareMathOperator*{\Exp}{\ensuremath{{\mathbb{E}}}}
\DeclareMathOperator*{\Prob}{\ensuremath{\mathbb{P}}}
\renewcommand{\Pr}{\Prob}
\newcommand{\EX}{\Exp}
\newcommand{\Ex}{\Exp}
\newcommand{\bigO}[1]{\ensuremath{O\Paren{#1}}}

\newcommand{\etal}{{\it et al.\,}}
\newcommand{\goodetal}{{\it et al.\/}}

% Paper:
\newcommand{\FF}{\ensuremath{\mathcal{F}}}
\newcommand{\FG}{\ensuremath{\mathcal{G}}}
\newcommand{\FV}{\ensuremath{\mathcal{V}}}
\newcommand{\FE}{\ensuremath{\mathcal{E}}}
\newcommand{\FM}{\ensuremath{\mathcal{M}}}

\newcommand{\odd}{\ensuremath{odd}}

\newcommand{\hM}{\ensuremath{\widehat{M}}}
\newcommand{\event}{\ensuremath{{\mathcal{E}}}}


\newcommand{\rs}{Ruzsa-Szemer\'{e}di\xspace}

%\newcommand{\evt}{\ensuremath{{\mathcal E}}}
\newcommand{\evt}{\ensuremath{{\sf E}}}
\newcommand{\Union}{\ensuremath{\bigcup}}

\newcommand{\tOPT}{\ensuremath{\widehat{\OPT}}}


\newcommand{\bMatch}{\ensuremath{\floor{{1 \over p}}}}

% Table: 
\newenvironment{tbox}{\begin{tcolorbox}[
		enlarge top by=5pt,
		enlarge bottom by=5pt,
		 breakable,
		 boxsep=0pt,
                  left=4pt,
                  right=4pt,
                  top=10pt,
                  arc=0pt,
                  boxrule=1pt,toprule=1pt,
                  colback=white
                  ]%%
	}
{\end{tcolorbox}}



%-------------------------- Textbox ---------------------------------

\newcommand{\textbox}[2]{
{
\begin{tbox}
\textbf{#1}
{#2}
\end{tbox}
}
}

%-------------------------- Paper ---------------------------------

\newcommand{\sign}{\ensuremath{\textnormal{sign}}\xspace}
\newcommand{\supp}{\ensuremath{\textnormal{supp}}\xspace}

\newcommand{\bx}{\ensuremath{\bm{x}}}

\newcommand{\QQ}{\mathbb{R}}
\newcommand{\calC}{{\cal C}}
\newcommand{\ProblemOne}{{Single Element Recovery}\xspace}
%\newcommand{\ProblemTwo}{${\mathsf{SupportHitter}^{\oplus L}}$}
%\newcommand{\ProblemThree}{$\mathsf{SpanningForest~}$}
\newcommand{\ALGO}{\mathscr{A}}

\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bh}{\boldsymbol{h}}


\newcommand{\heps}{\ensuremath{\widehat{\eps}}}
\newcommand{\TL}{\ensuremath{T}}

\newcommand{\alphalarge}{\ensuremath{\alpha}_{\textnormal{\textsf{large}}}}
\newcommand{\betaheavy}{\ensuremath{\beta}_{\textnormal{\textsf{heavy}}}}


\newcommand{\adv}{\ensuremath{\textsc{adversary}}\xspace}

\newcommand{\Qk}{\ensuremath{Q^{(k)}}}

==> prelim.tex <==
% !TeX root = main.tex 
%!TEX root = main.tex

\section{Notations}\label{sec:prelim}

Throughout the paper, for a positive integer $N$, we use $[N]$ to denote the set $\{1,2,\ldots, N\}$.
Whenever we use the term ``with high probability'' or whp, we mean with probability $\geq 1 - \frac{1}{\poly(n)}$, where $n$ is the relevant size parameter.

Given a multigraph $G$, given two disjoint subsets of  vertices $S,T \subseteq V$, we let $E(S,T)$ denote the collection of {\em pairs} $(u,v)$ with $u\in S, v\notin S$ such that there is at least one edge
between $u$ and $v$. 


